Updated determination of $D^0$-$\overline{D}{}^0$ mixing and CP violation parameters with $D^0\to K^+\pi^-$ decays

We report measurements of charm-mixing parameters based on the decay-time-dependent ratio of $D^0\to K^+\pi^-$ to $D^0\to K^-\pi^+$ rates. The analysis uses a data sample of proton-proton collisions corresponding to an integrated luminosity of $5.0$ fb$^{-1}$ recorded by the LHCb experiment from 2011 through 2016. Assuming charge-parity (CP) symmetry, the mixing parameters are determined to be $x'^2=(3.9 \pm 2.7) \times10^{-5}$, $y'=(5.28 \pm 0.52) \times 10^{-3}$, and $R_D=(3.454 \pm 0.031)\times10^{-3}$. Without this assumption, the measurement is performed separately for $D^0$ and $\overline{D}{}^0$ mesons, yielding a direct CP-violating asymmetry $A_D =(-0.1\pm9.1)\times10^{-3}$, and magnitude of the ratio of mixing parameters $1.00< |q/p| <1.35$ at the $68.3\%$ confidence level. All results include statistical and systematic uncertainties and improve significantly upon previous single-measurement determinations. No evidence for CP violation in charm mixing is observed.

==> LHCb_Authorship_flat_19-Oct-2017/LHCb_Authorship_flat_arXiv_19-Oct-2017.tex <==
LHCb collaboration: 
R. Aaij,
B. Adeva,
M. Adinolfi,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
S. Ali,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
S. Amerio,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
J.E. Andrews,
R.B. Appleby,
F. Archilli,
P. d'Argent,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
E. Aslanides,
M. Atzeni,
G. Auriemma,
M. Baalouch,
I. Babuschkin,
S. Bachmann,
J.J. Back,
A. Badalov,
C. Baesso,
S. Baker,
V. Balagura,
W. Baldini,
A. Baranov,
R.J. Barlow,
C. Barschel,
S. Barsuk,
W. Barter,
F. Baryshnikov,
V. Batozskaya,
V. Battista,
A. Bay,
L. Beaucourt,
J. Beddow,
F. Bedeschi,
I. Bediaga,
A. Beiter,
L.J. Bel,
N. Beliy,
V. Bellee,
N. Belloli,
K. Belous,
I. Belyaev,
E. Ben-Haim,
G. Bencivenni,
S. Benson,
S. Beranek,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.O. Bettler,
M. van Beuzekom,
Ia. Bezshyiko,
S. Bifani,
P. Billoir,
A. Birnkraut,
A. Bizzeti,
M. Bj{\o}rn,
T. Blake,
F. Blanc,
S. Blusk,
V. Bocci,
T. Boettcher,
A. Bondar,
N. Bondar,
I. Bordyuzhin,
S. Borghi,
M. Borisyak,
M. Borsato,
F. Bossu,
M. Boubdir,
T.J.V. Bowcock,
E. Bowen,
C. Bozzi,
S. Braun,
J. Brodzicka,
D. Brundu,
E. Buchanan,
C. Burr,
A. Bursche,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carson,
K. Carvalho Akiba,
G. Casse,
L. Cassina,
M. Cattaneo,
G. Cavallero,
R. Cenci,
D. Chamont,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
S. Chen,
S.F. Cheung,
S.-G. Chitic,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
V. Coco,
J. Cogan,
E. Cogneras,
V. Cogoni,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
A. Contu,
G. Coombs,
S. Coquereau,
G. Corti,
M. Corvo,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
R. Currie,
C. D'Ambrosio,
F. Da Cunha Marinho,
C.L. Da Silva,
E. Dall'Occo,
J. Dalseno,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
C.T. Dean,
D. Decamp,
L. Del Buono,
H.-P. Dembinski,
M. Demmer,
A. Dendek,
D. Derkach,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Canto,
P. Di Nezza,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A. Dosil Su{\'a}rez,
L. Douglas,
A. Dovbnya,
K. Dreimanis,
L. Dufour,
G. Dujany,
P. Durante,
J.M. Durham,
D. Dutta,
R. Dzhelyadin,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
M. Ebert,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
U. Eitschberger,
R. Ekelhof,
L. Eklund,
S. Ely,
S. Esen,
H.M. Evans,
T. Evans,
A. Falabella,
N. Farley,
S. Farry,
D. Fazzini,
L. Federici,
D. Ferguson,
G. Fernandez,
P. Fernandez Declara,
A. Fernandez Prieto,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Frank,
C. Frei,
J. Fu,
W. Funk,
E. Furfaro,
C. F{\"a}rber,
E. Gabriel,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
J. Garc{\'\i}a Pardi{\~n}as,
J. Garra Tico,
L. Garrido,
D. Gascon,
C. Gaspar,
L. Gavardi,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
Ph. Ghez,
S. Gian{\`\i},
V. Gibson,
O.G. Girard,
L. Giubega,
K. Gizdov,
V.V. Gligorov,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
R. Greim,
P. Griffith,
L. Grillo,
L. Gruber,
B.R. Gruberg Cazon,
O. Gr{\"u}nberg,
E. Gushchin,
Yu. Guz,
T. Gys,
C. G{\"o}bel,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
B. Hamilton,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
S.T. Harnew,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heinicke,
A. Heister,
K. Hennessy,
P. Henrard,
L. Henry,
E. van Herwijnen,
M. He{\ss},
A. Hicheur,
D. Hill,
P.H. Hopchev,
W. Hu,
W. Huang,
Z.C. Huard,
W. Hulsbergen,
T. Humair,
M. Hushchyn,
D. Hutchcroft,
P. Ibis,
M. Idzik,
P. Ilten,
R. Jacobsson,
J. Jalocha,
E. Jans,
A. Jawahery,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
C. Joram,
B. Jost,
N. Jurik,
S. Kandybei,
M. Karacson,
J.M. Kariuki,
S. Karodia,
N. Kazeev,
M. Kecke,
F. Keizer,
M. Kelsey,
M. Kenzie,
T. Ketel,
E. Khairullin,
B. Khanji,
C. Khurewathanakul,
T. Kirn,
S. Klaver,
K. Klimaszewski,
T. Klimkovich,
S. Koliiev,
M. Kolpin,
I. Komarov,
R. Kopecna,
P. Koppenburg,
A. Kosmyntseva,
S. Kotriakhova,
M. Kozeiha,
L. Kravchuk,
M. Kreps,
F. Kress,
P. Krokovny,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
A.K. Kuonen,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
C. Lazzeroni,
R. Le Gac,
A. Leflat,
J. Lefran{\c{c}}ois,
R. Lef{\`e}vre,
F. Lemaitre,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
B. Leverington,
P.-R. Li,
T. Li,
Y. Li,
Z. Li,
X. Liang,
T. Likhomanenko,
R. Lindner,
F. Lionetto,
V. Lisovskyi,
X. Liu,
D. Loh,
A. Loi,
I. Longstaff,
J.H. Lopes,
D. Lucchesi,
M. Lucio Martinez,
H. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Maev,
K. Maguire,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
G. Martellotti,
M. Martin,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
R. Matev,
A. Mathad,
Z. Mathe,
C. Matteuzzi,
A. Mauri,
E. Maurice,
B. Maurin,
A. Mazurov,
M. McCann,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
F. Meier,
N. Meinert,
D. Melnychuk,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
E. Millard,
M.-N. Minard,
L. Minzoni,
D.S. Mitzel,
A. Mogini,
J. Molina Rodriguez,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
M.J. Morello,
O. Morgunova,
J. Moron,
A.B. Morris,
R. Mountain,
F. Muheim,
M. Mulder,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
M. Neuner,
T.D. Nguyen,
C. Nguyen-Mau,
S. Nieswand,
R. Niet,
N. Nikitin,
T. Nikodem,
A. Nogay,
D.P. O'Hanlon,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
R. Oldeman,
C.J.G. Onderwater,
A. Ossowska,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
P.R. Pais,
A. Palano,
M. Palutan,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
M. Petruzzo,
E. Picatoste Olloqui,
B. Pietrzyk,
G. Pietrzyk,
M. Pikies,
D. Pinci,
F. Pisani,
A. Pistone,
A. Piucci,
V. Placinta,
S. Playfer,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
A. Poluektov,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
A. Popov,
D. Popov,
S. Poslavskii,
C. Potterat,
E. Price,
J. Prisciandaro,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
H. Pullen,
G. Punzi,
W. Qian,
J. Qin,
R. Quagliani,
B. Quintana,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
I. Raniuk,
F. Ratnikov,
G. Raven,
M. Ravonel Salzgeber,
M. Reboud,
F. Redi,
S. Reichert,
A.C. dos Reis,
C. Remon Alepuz,
V. Renaudin,
S. Ricciardi,
S. Richards,
M. Rihl,
K. Rinnert,
P. Robbe,
A. Robert,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
A. Rogozhnikov,
S. Roiser,
A. Rollings,
V. Romanovskiy,
A. Romero Vidal,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
P. Ruiz Valls,
J. Ruiz Vidal,
J.J. Saborido Silva,
E. Sadykhov,
N. Sagidova,
B. Saitta,
V. Salustino Guimaraes,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
G. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
D.M. Saunders,
D. Savrina,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
H.F. Schreiner,
M. Schubiger,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
A. Semennikov,
E.S. Sepulveda,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
P. Seyfert,
M. Shapkin,
I. Shapoval,
Y. Shcheglov,
T. Shears,
L. Shekhtman,
V. Shevchenko,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
M. Sirendi,
N. Skidmore,
T. Skwarnicki,
I.T. Smith,
J. Smith,
M. Smith,
l. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
P. Spradlin,
S. Sridharan,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
M. Stepanova,
H. Stevens,
S. Stone,
B. Storaci,
S. Stracka,
M.E. Stramaglia,
M. Straticiuc,
U. Straumann,
J. Sun,
L. Sun,
K. Swientek,
V. Syropoulos,
T. Szumlak,
M. Szymanski,
S. T'Jampens,
A. Tayduganov,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
J. van Tilburg,
M.J. Tilley,
V. Tisserand,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
R. Tourinho Jadallah Aoude,
E. Tournefier,
M. Traill,
M.T. Tran,
M. Tresch,
A. Trisovic,
A. Tsaregorodtsev,
P. Tsopelas,
A. Tully,
N. Tuning,
A. Ukleja,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
C. Vacca,
A. Vagner,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
R. Vazquez Gomez,
P. Vazquez Regueiro,
S. Vecchi,
M. van Veghel,
J.J. Velthuis,
M. Veltri,
G. Veneziano,
A. Venkateswaran,
T.A. Verlage,
M. Vernet,
M. Veronesi,
M. Vesterinen,
J.V. Viana Barbosa,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
M. Vitti,
V. Volkov,
A. Vollhardt,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
C. Vo{\ss},
J.A. de Vries,
C. V{\'a}zquez Sierra,
R. Waldi,
J. Walsh,
J. Wang,
Y. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
C. Weisser,
M. Whitehead,
J. Wicht,
G. Wilkinson,
M. Wilkinson,
M. Williams,
M. Williams,
T. Williams,
F.F. Wilson,
J. Wimberley,
M. Winn,
J. Wishahi,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
K. Wyllie,
Y. Xie,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
Z. Yang,
Z. Yang,
Y. Yao,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
L. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli
